ImDrug: A Benchmark for Deep Imbalanced Learning in AI-aided Drug Discovery

The last decade has witnessed a prosperous development of computational methods and dataset curation for AI-aided drug discovery (AIDD). However, real-world pharmaceutical datasets often exhibit highly imbalanced distribution, which is overlooked by the current literature but may severely compromise the fairness and generalization of machine learning applications. Motivated by this observation, we introduce ImDrug, a comprehensive benchmark with an open-source Python library which consists of 4 imbalance settings, 11 AI-ready datasets, 54 learning tasks and 16 baseline algorithms tailored for imbalanced learning. It provides an accessible and customizable testbed for problems and solutions spanning a broad spectrum of the drug discovery pipeline such as molecular modeling, drug-target interaction and retrosynthesis. We conduct extensive empirical studies with novel evaluation metrics, to demonstrate that the existing algorithms fall short of solving medicinal and pharmaceutical challenges in the data imbalance scenario. We believe that ImDrug opens up avenues for future research and development, on real-world challenges at the intersection of AIDD and deep imbalanced learning.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> Tables-new/table-2-new-copy.tex <==
% \begin{wraptable}{r}{9cm}
% \small
% \centering
% \vspace{-2em}
% \caption{\textbf{Results on Open LT.} The proportions of samples split into open-sets in USPTO-50K and DrugBank are 0.2 and 0.5, respectively.}\label{table:openLT}
% % For each dataset and metric, the best method is bolded and the second best is underlined.
% \vspace{1em}
% \scalebox{0.6}{
% \begin{tabular}{c|ccc|cll}
% \toprule
%                   & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
%                   & Balanced-Acc & Balanced-F1 & AUROC     & balanced-acc & \multicolumn{1}{c}{balanced-f1} & \multicolumn{1}{c}{AUROC} \\ \midrule
% Vanilla GCN      & $37.52_{\pm0.45}$   & $35.04_{\pm0.64}$  & $73.66_{\pm0.26}$ & $58.29_{\pm0.56}$   & $62.46_{\pm0.42}$                      & $96.94_{\pm0.27}$                  \\\midrule
% BS & $39.54_{\pm0.99}$   & $37.03_{\pm1.27}$  & $73.66_{\pm0.59}$  & $71.12_{\pm0.27}$   & $71.60_{\pm0.28}$                      & $97.34_{\pm0.27}$                  \\
% CB\_F & $37.28_{\pm1.36}$   & $34.62_{\pm0.71}$  & $71.94_{\pm0.65}$  & $59.75_{\pm0.39}$   & $63.26_{\pm0.78}$                      & $96.54_{\pm0.09}$                  \\
% Remix             & $48.28_{\pm0.41}$   & $45.05_{\pm0.46}$  & $76.23_{\pm0.65}$  & $69.78_{\pm0.71}$   & $72.72_{\pm0.61}$                     & $97.68_{\pm0.07}$                  \\
% IB & $39.62_{\pm0.99}$   & $33.55_{\pm2.2}$   & $69.86_{\pm0.88}$  & $62.81_{\pm0.96}$   & $64.00_{\pm0.64}$                     & $94.67_{\pm0.23}$                  \\
% BBN               & $51.30_{\pm0.35}$   & $47.82_{\pm0.31}$  & $77.05_{\pm0.29}$  & $78.75_{\pm0.52}$   & $79.36_{\pm0.25}$                      & $97.32_{\pm0.08}$                  \\ \midrule
% OLTR         & ${50.12_{\pm0.55}}$   & $47.24_{\pm0.40}$  & ${79.76_{\pm0.22}}$  & $73.55_{\pm0.34}$   & $73.54_{\pm0.29}$                      & $97.23_{\pm0.66}$                  \\
% IEM          & $51.63_{\pm0.59}$   & $48.23_{\pm0.50}$  & $\underline{80.91_{\pm0.52}}$  & $75.67_{\pm0.76}$   & $76.63_{\pm0.43}$                      & $\boldsymbol{98.09_{\pm0.23}}$                  \\ 
% OLTR+BBN   &            $\boldsymbol{60.39_{\pm0.51}}$     &  $\boldsymbol{56.09_{\pm5.20}}$                  &    $\boldsymbol{85.27_{\pm2.16}}$                            &              $\boldsymbol{82.56_{\pm5.89}}$                   &               $\boldsymbol{82.47_{\pm0.40}}$                 &                     $\underline{97.78_{\pm7.99}}$                                                                                       \\
% IEM+BBN    &          $\underline{58.63_{\pm0.42}}$                           &         $\underline{53.26_{\pm0.44}}$                       &           $80.10_{\pm3.62}$                      &            $\underline{81.80_{\pm0.67}}$                    &                  $\underline{82.13_{\pm0.46}}$                                  &    $97.58_{\pm0.53}$                                                    \\
% \bottomrule
% \end{tabular}
% }
% \end{wraptable}



\begin{table}[t]
\parbox{.58\linewidth}{
      \caption{\textbf{Results on Open LT \textcolor{blue}{under random split}.} The proportions of samples split into open-sets in USPTO-50K~\textcolor{blue}{(single-instance prediction)} and DrugBank~\textcolor{blue}{(multi-instance prediction)} are 0.2 and 0.5, respectively.}\label{table:openLT}
\begin{adjustbox}{max width=.58\textwidth}
  \centering
\begin{tabular}{c|ccc|cll}
\toprule
                  & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
                  & Balanced-Acc & Balanced-F1 & AUROC     & Balanced-Acc & \multicolumn{1}{c}{Balanced-F1} & \multicolumn{1}{c}{AUROC} \\ \midrule
Vanilla GCN      & $85.82_{\pm0.42}$   & $81.38_{\pm0.41}$  & $94.18_{\pm0.066}$ & $91.72_{\pm0.28}$   & $91.75_{\pm0.33}$                      & $99.07_{\pm0.015}$                  \\\midrule
BS & $85.88_{\pm1.02}$   & $81.44_{\pm0.90}$  & $94.22_{\pm0.68}$  & $94.71_{\pm0.044}$   & $94.14_{\pm0.05}$                      & $99.11_{\pm0.03}$                  \\
CB\_F & $86.77_{\pm0.99}$   & $82.2_{\pm1.22}$  & $94.16_{\pm0.08}$  & $93.17_{\pm0.43}$   & $92.84_{\pm0.40}$                      & $98.80_{\pm0.11}$                  \\
Remix             & $87.92_{\pm0.23}$   & $83.40_{\pm0.21}$  & $93.91_{\pm0.13}$  & $92.68_{\pm0.83}$   & $92.75_{\pm0.59}$                     & $99.59_{\pm0.40}$                  \\
IB & $86.06_{\pm1.14}$   & $81.63_{\pm1.09}$   & $94.15_{\pm0.040}$  & $92.95_{\pm0.31}$   & $92.31_{\pm0.31}$                     & $99.03_{\pm0.04}$                  \\
BBN               & $87.86_{\pm0.14}$   & $83.32_{\pm0.13}$  & $94.07_{\pm0.19}$  & $94.52_{\pm0.33}$   & $93.96_{\pm0.34}$                      & $98.92_{\pm0.07}$                  \\ \midrule
OLTR         & ${89.21_{\pm0.75}}$   & $85.11_{\pm0.38}$  & ${96.69_{\pm0.12}}$  & $95.37_{\pm0.30}$   & $94.92_{\pm0.16}$                      & $\boldsymbol{99.79_{\pm0.09}}$                  \\
IEM          & $89.99_{\pm0.29}$   & $85.46_{\pm0.20}$  & $\underline{96.74_{\pm0.09}}$  & $95.77_{\pm0.16}$   & $95.16_{\pm0.15}$                      & $99.64_{\pm0.08}$                  \\ 
OLTR+BBN   &            $\boldsymbol{91.18_{\pm0.11}}$     &  $\boldsymbol{87.97_{\pm0.60}}$                  &    $\boldsymbol{97.72_{\pm0.56}}$                            &              $\boldsymbol{96.84_{\pm1.59}}$                   &               $\boldsymbol{96.12_{\pm0.93}}$                 &                     $\boldsymbol{99.89_{\pm0.69}}$                                                                                       \\
IEM+BBN    &          $\underline{90.66_{\pm0.41}}$                           &         $\underline{86.03_{\pm0.75}}$                       &           $96.64_{\pm1.03}$                      &            $\underline{96.06_{\pm0.76}}$                    &                  $\underline{95.59_{\pm0.96}}$                                  &    $99.77_{\pm0.12}$                                                    \\
\bottomrule
\end{tabular}
\end{adjustbox}
}
  \parbox{.42\linewidth}{
    % \vspace{0.2em}
       \caption{\textbf{Results on imbalanced regression \textcolor{blue}{under standard split}.} We report the average performance on SBAP-Reg~\textcolor{blue}{(multi-instance prediction)} and QM9~\textcolor{blue}{(single-instance prediction)} in terms of mean MSE and MAE with standard deviation in this setting.}
       \label{table:ImbalancedRegression}
      \begin{adjustbox}{max width=.4\textwidth}
      \centering 
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.66_{\pm1.03}$           & $0.92_{\pm0.25}$            & $76.17_{\pm42.82}$        & $6.57_{\pm1.92}$          \\
Mixup        & $\underline{1.10_{\pm0.51}}$           & $\underline{0.78_{\pm0.17}}$            &  $82.35_{\pm36.86}$       & $6.59_{\pm1.46}$                        \\
BBN          & $1.52_{\pm1.57}$           & $0.89_{\pm0.38}$            & $\underline{59.42_{\pm14.39}}$        & $6.02_{\pm0.77}$          \\ \midrule
Focal-R       & $1.38_{\pm1.08}$           & $0.84_{\pm0.31}$            & $94.29_{\pm57.38}$        & $7.23_{\pm2.65}$          \\
LDS          & $1.36_{\pm1.16}$           & $\underline{0.78_{\pm0.26}}$            & $\boldsymbol{16.01_{\pm6.58}}$        & $\boldsymbol{2.73_{\pm0.03}}$           \\
FDS          & $\boldsymbol{0.59_{\pm0.09}}$           & $\boldsymbol{0.54_{\pm0.02}}$            & $60.81_{\pm33.52}$        & $\underline{5.63_{\pm1.53}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
}
\end{table}

==> Tables-new/table-4-new.tex <==
% \begin{wraptable}[9]{r}{7.5cm}
\begin{table}[tbh]
\vspace{-2em}
\caption{\textbf{Results on imbalanced regression.} }\label{table:ImbalancedRegression}
\vspace{1em}
\small
\centering
\begin{adjustbox}{max width=0.5\textwidth}
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.99_{\pm0.52}$           & $1.13_{\pm0.14}$            & $161.55_{\pm38.18}$        & $10.40_{\pm1.39}$          \\
Mixup        & $1.34_{\pm0.18}$           & $0.92_{\pm0.17}$            &  $160.32_{\pm39.58}$       & $10.17_{\pm1.27}$                        \\
BBN          & $1.58_{\pm0.59}$           & $1.04_{\pm0.18}$            & $161.22_{\pm37.55}$        & $10.04_{\pm1.13}$          \\ \midrule
Focal\_R       & $1.92_{\pm0.69}$           & $1.14_{\pm0.30}$            & $171.78_{\pm40.60}$        & $10.70_{\pm1.16}$          \\
LDS          & $\underline{1.11_{\pm0.16}}$           & $\boldsymbol{0.67_{\pm0.01}}$            & $\underline{143.15_{\pm20.69}}$        & $\underline{9.63_{\pm0.72}}$           \\
FDS          & $\boldsymbol{0.85_{\pm0.08}}$           & $\underline{0.71_{\pm0.12}}$            & $\boldsymbol{134.83_{\pm41.61}}$        & $\boldsymbol{9.28_{\pm1.51}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \end{wraptable}

==> Tables/Loss_functions.tex <==
\begin{wraptable}[15]{r}{0.6\linewidth}
% \vspace*{-\baselineskip}
\centering
\caption{\textbf{Summary of re-balancing losses.} $z$ and $p$ denote the predicted logits and the softmax probability of the sample $x$, with subscript $y$ being the corresponding class label. $n_y$ and $\pi_y$ indicate the sample number and label frequency of the class $y$. $\gamma$ and $\beta$ are loss-related hyperparameters.}
\renewcommand{\arraystretch}{1.5}
\label{table:loss_functions}
\vspace{1em}
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{max width=0.6\textwidth}
\begin{tabular}{ll}
\toprule
Losses & Formulation \\ \midrule
Softmax loss (vanilla) & $\mathcal{L}_{CE} = -\log(p_y)$\\
Cost-sensitive loss~\cite{CostSensitiveCE} & $\mathcal{L}_{CS} =  -\frac{1}{\pi_y}\log(p_y)$\\
Class-balanced focal loss~\cite{ClassBalanceFocal} & $\mathcal{L}_{CB\_F} = -\frac{1-\gamma}{1-\gamma^{n_y}}(1-p_y)^{\beta}\log(p_y)$\\
Class-balanced cross-entropy loss~\cite{ClassBalanceFocal} & $\mathcal{L}_{CB\_CE} = -\frac{1-\gamma}{1-\gamma^{n_y}}\log(p_y) $\\
Balanced softmax loss~\cite{BalancedSoftmaxCE} & $\mathcal{L}_{BS} = -\log\left(\frac{\pi_y\exp(z_y)}{\sum_j\pi_j\exp(z_j)}\right)$\\
Influence-balanced loss~\cite{park2021influence} & $\mathcal{L}_{IB} = -\frac{1}{\pi_y||\nabla\log(p_y)||_1}\log(p_y)$\\
\bottomrule
% \vspace*{-0.15in}
\end{tabular}
\end{adjustbox}
% \vspace*{-\baselineskip}
\end{wraptable}



==> Tables/table-1-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\small
\centering
\caption{\textbf{Results for random and standard splits on 4 ImDrug classification datasets.} We perform binary classification on HIV and SBAP, and long-tailed classification on USPTO-50K and DrugBank. For each split and metric, the best method is \textbf{bolded} and the second best is \underline{underlined}.}\label{table:overall}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccc|ccc|ccc|ccc|ccc}
\toprule
                                        \multicolumn{3}{c}{}  & \multicolumn{3}{c}{\textbf{HIV}\cite{wu2018moleculenet}}                                                                        & \multicolumn{3}{c}{\textbf{SBAP}\cite{2022arXiv220109637J}}         & \multicolumn{3}{c}{\textbf{USPTO-50K}\cite{liu2017retrosynthetic}}    & \multicolumn{3}{c}{\textbf{DrugBank}\cite{wishart2018drugbank}}     \\\midrule
\multicolumn{3}{c}{\# Graphs}                        & \multicolumn{3}{c}{41,127}                                                                     & \multicolumn{3}{c}{32,140}             & \multicolumn{3}{c}{50,036}             & \multicolumn{3}{c}{191,808}             \\
\multicolumn{3}{c}{\# Average nodes}                & \multicolumn{3}{c}{25.51}                                                                      & \multicolumn{3}{c}{32.60}             & \multicolumn{3}{c}{25.03}             & \multicolumn{3}{c}{26.43}             \\
\multicolumn{3}{c}{\# Average edges}         & \multicolumn{3}{c}{54.94}                                                                      & \multicolumn{3}{c}{103.94}             & \multicolumn{3}{c}{78.29}             & \multicolumn{3}{c}{83.21}             \\
\multicolumn{3}{c}{\# Classes}            & \multicolumn{3}{c}{2}                                                                          & \multicolumn{3}{c}{2}             & \multicolumn{3}{c}{10}             & \multicolumn{3}{c}{86}  \\           
\multicolumn{3}{c}{Imbalance ratio}            & \multicolumn{3}{c}{27.50}                                                                          & \multicolumn{3}{c}{36.77}             & \multicolumn{3}{c}{65.78}             & \multicolumn{3}{c}{216.96} 
\\ \midrule\midrule
\multicolumn{3}{c|}{Metric}                                                                                         & Balanced-Acc                          & Balanced-F1                           & AUROC            & Balanced-Acc & Balanced-F1 & AUROC & Balanced-Acc & Balanced-F1 & AUROC & Balanced-Acc & Balanced-F1 & AUROC \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Vanilla GCN       & 71.89                        & 69.82                         & 83.03 &  77.50            &     76.39        &  95.07   & 92.23      & 92.20            & 99.76     & 87.54     & 87.60     & 99.78      \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & BS  & \textbf{77.13}                        & \textbf{76.71}                        & \textbf{83.91} &   83.21          &      83.06       &  91.01   & 93.69     & 93.71    & 99.76      & \textbf{94.98}    & \textbf{94.77}          &  99.60   \\
\multicolumn{1}{c|}{}                            &                                            & CB\_F  & 73.14                        & 72.66                        & 82.23 &    81.02         &      79.88       &  94.59   & 93.32     & 93.33    & 99.49      & 93.71    & 93.79          &  99.31   \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Class- \\ rebalancing\end{tabular}}        & CS    & \underline{77.04}                        & \underline{76.66}                        & 79.90 &        \textbf{91.49}      &      \textbf{91.48}       & \textbf{96.67}   & 93.01     & 93.04    & 99.71      & 93.67    & 93.70       & 99.39     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & Mixup              & 73.06                       & 70.62                        & 82.99 &           78.38   &      77.41       &  95.81   & \underline{95.03}     & \underline{95.04}    & \underline{99.77}      & 92.15            & 91.78             &  \textbf{99.84}    \\
\multicolumn{1}{c|}{}                            &                                            & Remix              & 74.43                        & 72.19                        & 81.09 &    79.58          &      78.49       &  95.01   & 94.83     & 94.84    & 95.26     & 94.47              & \underline{94.32}             & 99.76     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Information \\augmentation\end{tabular}} & DiVE               & 75.07 & 74.24 & 81.12 &         84.58     &        84.65     &   95.43    & 93.90      &  93.91           & 99.60     & 90.26 & 91.08 & 99.42  \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & CDT                & 71.67                        & 69.52                         & 82.95 &        78.92      &     78.17        &  95.58   & 93.92     & 93.92   & \textbf{99.78} & \underline{94.54}              & \underline{94.32}             & 99.52     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & 74.64 &  73.33 & \underline{83.66} &      85.04        &       84.82      &    95.66 &  92.81        & 92.81           & 94.43     &  90.00   &  90.27           & \underline{99.79}     \\
\multicolumn{1}{c|}{}                            &                                            & IB & 73.80                        &         71.32                & 79.88 &         83.70     &      83.61       &  90.65   & 93.00      & 93.00   & 99.66     & 90.38              & 90.10             & 99.39     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Random}}   & \multirow{-4}{*}{\begin{tabular}{c}Module \\Improvement\end{tabular}}       & BBN                & 76.50                        & 76.36                        & 81.65 &       \underline{90.67}       &      \underline{90.67}       &   \underline{96.16}  & \textbf{95.57}      & \textbf{95.56}   & 99.67   &  92.55             & 92.54             & 99.48     \\ \midrule\midrule
\multicolumn{1}{c|}{}                            &                                            & Vanilla GCN       & 71.24                        & 68.99                        & 80.99 &    77.29          &  76.21           &  94.70   &  92.15      & 92.15  & 99.54   & 89.38              &    86.96         & 98.09     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & BS  & 75.04                        & 74.85                        & 79.60 &     88.41         &      88.38       &  \underline{95.16}   & 93.62    & 93.59  & 99.63    & \underline{94.69}             & 92.58            & \underline{98.93}     \\
\multicolumn{1}{c|}{}                            &                                            & CB\_F  & 71.57                       & 69.57                    & 80.59 &         84.70     &       83.78      &  94.93     & 94.07  & 94.11  & 99.27  &   90.55           & 88.09             & 97.77     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Class- \\rebalancing\end{tabular}}        & CS    & \textbf{76.95}                        & \textbf{76.39}                        & 81.06 &  \textbf{89.79}            &      \textbf{89.78}      & \textbf{95.61}   &  92.73  & 92.76 & 99.62 &   \underline{94.69}         & \underline{92.89}             & 98.50     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & Mixup              & 71.48                        & 69.31                        &  \underline{81.18} &      79.69       &      78.04       &   94.99  &  95.21      & 95.19 & \underline{99.65} &  85.45            & 83.48             & \textbf{99.13}     \\
\multicolumn{1}{c|}{}                            &                                            & Remix              & 71.59                        & 69.47                        & \textbf{81.53} &      77.90        &      76.71       & 94.56    & \underline{95.27}       & \underline{95.25} & 99.57     & 89.93              & 87.46             & 98.78     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Information \\augmentation\end{tabular}} & DiVE               &  74.16 &  72.69 & 81.06 &   86.69           &      86.65       & 93.41    &    94.03      & 94.00     & 99.43     & 89.95  & 87.46 & 98.33 \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & CDT                & 71.87                       & 68.94                        & 80.47 &       81.51       &       80.98      &    94.14  & 93.79      & 93.78 & \underline{99.65}   &  91.15         & 88.29             & 98.80     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & 73.14                        & 71.52                        & 80.00 &       69.58       &      66.33       &   90.99  &  92.64      & 92.60 & 99.56    & 89.97        & 87.30       & 98.61    \\
\multicolumn{1}{c|}{}                            &                                            & IB &  \underline{75.34} &  \underline{75.14} & 80.16 &     84.87         &       84.87      &    91.41  & 91.51   & 91.55  & 98.90     &    89.98          & 87.14             &  98.39    \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Standard}} & \multirow{-4}{*}{\begin{tabular}{c}Module \\Improvement\end{tabular}}       & BBN                & 73.50                        & 73.39                        & 80.96 &        \underline{88.49}      &      \underline{88.45}       &  94.02   & \textbf{96.23}       & \textbf{96.25}  & \textbf{99.75}   & \textbf{95.28}             & \textbf{93.61}             & 98.52    \\ \bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-1em}
\end{table}

==> Tables/table-1-old-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\scalebox{0.8}{
\begin{tabular}{ccccccccccccccc}
\toprule
                                                 &                                            &                    & \multicolumn{3}{c}{HIV}                                                                        & \multicolumn{3}{c}{Sbap}         & \multicolumn{3}{c}{USPTO-50K}    & \multicolumn{3}{c}{DrugBank}     \\
\# Graphs                                        &                                            &                    & \multicolumn{3}{c}{41,127}                                                                     & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Average nodes                                 &                                            &                    & \multicolumn{3}{c}{25.51}                                                                      & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Average edges                                 &                                            &                    & \multicolumn{3}{c}{54.94}                                                                      & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Classes                                       &                                            &                    & \multicolumn{3}{c}{2}                                                                          & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\ \midrule
\multicolumn{3}{c}{Metric}                                                                                         & balanced-acc                          & balanced-f1                           & auc            & balanced-acc & balanced-f1 & auc & balanced-acc & balanced-f1 & auc & balanced-acc & balanced-f1 & auc \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Baseline-GCN       & 0.6277+-0.0169                        & 0.5739+-0.027                         & 0.7029+-0.0185 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & BalancedSoftmaxCE  & 0.7026+-0.0066                        & 0.6950+-0.0098                        & 0.7553+-0.0088 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & ClassBalanceFocal  & 0.6618+-0.0251                        & 0.6249+-0.0345                        & 0.7411+-0.0221 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Class-rebalancing}        & CostSensitiveCE    & 0.7010+-0.0095                        & 0.6892+-0.0097                        & 0.7433+-0.0050 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & mixup              & 0.6246+-0.0107                        & 0.5670+-0.0178                        & 0.7151+-0.0113 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & remix              & 0.6217+-0.0144                        & 0.5624+-0.0232                        & 0.7301+-0.0139 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Information augmentation} & DiVE               & {\color[HTML]{333333} 0.6869+-0.0127} & {\color[HTML]{333333} 0.6727+-0.0154} & 0.7221+-0.0117 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & CDT                & 0.6331+-0.0181                        & 0.5822+-0.027                         & 0.7289+-0.0215 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & {\color[HTML]{333333} 0.6943+-0.0087} & {\color[HTML]{333333} 0.6708+-0.0109} & 0.7445+-0.0131 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Influence Balanced & 0.6825+-0.0072                        & 0.6677+-0.0119                        & 0.7299+-0.0028 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Random}}   & \multirow{-4}{*}{Module Improvement}       & BBN                & 0.6822+-0.1266                        & 0.6304+-0.1783                        & 0.7298+-0.1509 &              &             &     &              &             &     &              &             &     \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Baseline-GCN       & 0.6308+-0.0121                        & 0.5801+-0.0162                        & 0.6852+-0.0127 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & BalancedSoftmaxCE  & 0.6730+-0.0047                        & 0.6643+-0.0034                        & 0.7211+-0.0096 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & ClassBalanceFocal  & 0.6539+-0.0073                        & 0.6143+-0.0099                        & 0.7498+-0.0141 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Class-rebalancing}        & CostSensitiveCE    & 0.6981+-0.0153                        & 0.6892+-0.0102                        & 0.7418+-0.0145 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & mixup              & 0.6310+-0.0135                        & 0.5775+-0.0206                        & 0.7240+-0.0176 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & remix              & 0.6371+-0.0079                        & 0.5864+-0.0097                        & 0.7278+-0.0274 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Information augmentation} & DiVE               & {\color[HTML]{333333} 0.6931+-0.0120} & {\color[HTML]{333333} 0.6890+-0.0126} & 0.7192+-0.0210 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & CDT                & 0.6315+-0.0103                        & 0.5802+-0.0133                        & 0.7133+-0.0177 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & 0.6864+-0.0064                        & 0.6622+-0.0092                        & 0.7338+-0.0096 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Influence Balanced & {\color[HTML]{333333} 0.6943+-0.0100} & {\color[HTML]{333333} 0.6821+-0.0103} & 0.7286+-0.0042 &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Standard}} & \multirow{-4}{*}{Module Improvement}       & BBN                & 0.6822+-0.1266                        & 0.6304+-0.1783                        & 0.7298+-0.1509 &              &             &     &              &             &     &              &             &     \\ \bottomrule
\end{tabular}
}
\end{table}

==> Tables/table-1-old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\caption{.}
\scalebox{0.3}{
\begin{tabular}{ccccccccccccccccccccc}
\toprule
                                                 &                                            &                    & \multicolumn{3}{c}{BBB}                          & \multicolumn{3}{c}{Tox21}                                               & \multicolumn{3}{c}{HIV}                                                                        & \multicolumn{3}{c}{Sbap}         & \multicolumn{3}{c}{USPTO-50K}    & \multicolumn{3}{c}{DrugBank}     \\\midrule
\# Graphs                                        &                                            &                    & \multicolumn{3}{c}{1,975}                        & \multicolumn{3}{c}{7,831}                                               & \multicolumn{3}{c}{41,127}                                                                     & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Average nodes                                 &                                            &                    & \multicolumn{3}{c}{24.06}                        & \multicolumn{3}{c}{18.57}                                               & \multicolumn{3}{c}{25.51}                                                                      & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Average edges                                 &                                            &                    & \multicolumn{3}{c}{51.91}                        & \multicolumn{3}{c}{38.59}                                               & \multicolumn{3}{c}{54.94}                                                                      & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\
\# Classes                                       &                                            &                    & \multicolumn{3}{c}{2}                            & \multicolumn{3}{c}{2}                                                   & \multicolumn{3}{c}{2}                                                                          & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             & \multicolumn{3}{c}{}             \\ \midrule\midrule
\multicolumn{3}{c}{Metric}                                                                                         & balanced-acc   & balanced-f1    & auc            & balanced-acc                          & balanced-f1    & auc            & balanced-acc                          & balanced-f1                           & auc            & balanced-acc & balanced-f1 & auc & balanced-acc & balanced-f1 & auc & balanced-acc & balanced-f1 & auc \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Baseline-GCN       & $0.6818_{\pm0.0114}$ & $0.6666_{\pm0.0164}$ & $0.7232_{\pm0.0146}$ & $0.6028_{\pm0.0337}$                        & $0.5325_{\pm0.0548}$ & $0.6271_{\pm0.0331}$ & $0.6277_{\pm0.0169}$                        & $0.5739_{\pm0.027}$                         & $0.7029_{\pm0.0185}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & BalancedSoftmaxCE  & $0.7030_{\pm0.0224}$ & $0.6969_{\pm0.0260}$ & $0.7584_{\pm0.0196}$ & $0.6793_{\pm0.0464}$                        & $0.6673_{\pm0.0543}$ & $0.6892_{\pm0.0490}$ & $0.7026_{\pm0.0066}$                        & $0.6950_{\pm0.0098}$                        & $0.7553_{\pm0.0088}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & ClassBalanceFocal  & $0.7038_{\pm0.0069}$ & $0.6946_{\pm0.0086}$ & $0.7572_{\pm0.0180}$ & $0.6434_{\pm0.0488}$                        & $0.6049_{\pm0.0665}$ & $0.6658_{\pm0.0655}$ & $0.6618_{\pm0.0251}$                        & $0.6249_{\pm0.0345}$                        & $0.7411_{\pm0.0221}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Class-rebalancing}        & CostSensitiveCE    & $0.6763_{\pm0.0083}$ & $0.6697_{\pm0.0062}$ & $0.7428_{\pm0.0034}$ & $0.6681_{\pm0.0160}$                        & $0.6549_{\pm0.0251}$ & $0.6765_{\pm0.0519}$ & $0.7010_{\pm0.0095}$                        & $0.6892_{\pm0.0097}$                        & $0.7433_{\pm0.0050}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & mixup              & $0.6750_{\pm0.0041}$ & $0.6593_{\pm0.0026}$ & $0.7189_{\pm0.0110}$ & $0.6249_{\pm0.0456}$                        & $0.5628_{\pm0.0678}$ & $0.6333_{\pm0.0369}$ & $0.6246_{\pm0.0107}$                        & $0.5670_{\pm0.0178}$                        & $0.7151_{\pm0.0113}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & remix              & $0.6796_{\pm0.0012}$ & $0.6625_{\pm0.0018}$ & $0.7415_{\pm0.0192}$ & $0.6200_{\pm0.0384}$                        & $0.5578_{\pm0.0595}$ & $0.6161_{\pm0.0309}$ & $0.6217_{\pm0.0144}$                        & $0.5624_{\pm0.0232}$                        & $0.7301_{\pm0.0139}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Information augmentation} & DiVE               & $0.703_{\pm0.0224}$  & $0.6969_{\pm0.026}$  & $0.7584_{\pm0.0196}$ & $0.6793_{\pm0.0464}$                        & $0.6673_{\pm0.0543}$ & $0.6892_{\pm0.049}$  & $0.6869_{\pm0.0127}$ & $0.6727_{\pm0.0154}$ & $0.7221_{\pm0.0117}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & CDT                & $0.7051_{\pm0.0233}$ & $0.6949_{\pm0.0294}$ & $0.7448_{\pm0.0267}$ & $0.5997_{\pm0.0153}$                        & $0.5271_{\pm0.0269}$ & $0.6547_{\pm0.0229}$ & $0.6331_{\pm0.0181}$                        & $0.5822_{\pm0.027}$                         & $0.7289_{\pm0.0215}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & $0.6937_{\pm0.0068}$ & $0.6816_{\pm0.0024}$ & $0.7482_{\pm0.012}$  & $0.6729_{\pm0.0352}$                        & $0.6434_{\pm0.0462}$ & $0.6794_{\pm0.0077}$ &  $0.6943_{\pm0.0087}$ &  $0.6708_{\pm0.0109}$ & $0.7445_{\pm0.0131}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Influence Balanced & $0.6797_{\pm0.0140}$ & $0.6620_{\pm0.0220}$ & $0.7445_{\pm0.0097}$ & $0.6542_{\pm0.0122}$                        & $0.6487_{\pm0.0099}$ & $0.7078_{\pm0.0003}$ & $0.6825_{\pm0.0072}$                        & $0.6677_{\pm0.0119}$                        & $0.7299_{\pm0.0028}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Random}}   & \multirow{-4}{*}{Module Improvement}       & BBN                & $0.6981_{\pm0.0213}$ & $0.6959_{\pm0.0201}$ & $0.7530_{\pm0.0176}$ & $0.6623_{\pm0.1293}$                        & $0.5980_{\pm0.1995}$ & $0.7533_{\pm0.1124}$ & $0.6822_{\pm0.1266}$                        & 0.6304_{\pm0.1783}$                        & 0.7298_{\pm0.1509}$ &              &             &     &              &             &     &              &             &     \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Baseline-GCN       & $0.7222_{\pm0.0120}$ & $0.7144_{\pm0.0145}$ & $0.7179_{\pm0.0121}$ & $0.6246_{\pm0.0068}$                        & $0.5674_{\pm0.0058}$ & $0.6272_{\pm0.0654}$ & $0.6308_{\pm0.0121}$                        & $0.5801_{\pm0.0162}$                        & $0.6852_{\pm0.0127}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & BalancedSoftmaxCE  & $0.6941_{\pm0.0109}$ & $0.6876_{\pm0.0103}$ & $0.7554_{\pm0.0135}$ & $0.6595_{\pm0.0433}$                        & $0.6493_{\pm0.0464}$ & $0.6882_{\pm0.0639}$ & $0.6730_{\pm0.0047}$                        & $0.6643_{\pm0.0034}$                        & $0.7211_{\pm0.0096}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & ClassBalanceFocal  & $0.7126_{\pm0.0360}$ & $0.7054_{\pm0.0399}$ & $0.7570_{\pm0.0206}$ & $0.6494_{\pm0.0164}$                        & $0.6111_{\pm0.0237}$ & $0.6900_{\pm0.0448}$ & $0.6539_{\pm0.0073}$                        & $0.6143_{\pm0.0099}$                        & $0.7498_{\pm0.0141}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Class-rebalancing}        & CostSensitiveCE    & $0.7397_{\pm0.0173}$ & $0.7367_{\pm0.0183}$ & $0.7841_{\pm0.0039}$ & $0.6760_{\pm0.0298}$                        & $0.6657_{\pm0.0288}$ & $0.6847_{\pm0.0491}$ & $0.6981_{\pm0.0153}$                        & $0.6892_{\pm0.0102}$                        & $0.7418_{\pm0.0145}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & mixup              & $0.7158_{\pm0.0218}$ & $0.7041_{\pm0.0243}$ & $0.7725_{\pm0.0199}$ & $0.5974_{\pm0.0219}$                        & $0.5238_{\pm0.0348}$ & $0.5971_{\pm0.0496}$ & $0.6310_{\pm0.0135}$                        & $0.5775_{\pm0.0206}$                        & $0.7240_{\pm0.0176}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & remix              & $0.7189_{\pm0.0055}$ & $0.7077_{\pm0.0063}$ & $0.7626_{\pm0.0150}$ & $0.6003_{\pm0.0054}$                        & $0.5288_{\pm0.0049}$ & $0.5974_{\pm0.0641}$ & $0.6371_{\pm0.0079}$                        & $0.5864_{\pm0.0097}$                        & $0.7278_{\pm0.0274}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{Information augmentation} & DiVE               & $0.6941_{\pm0.0109}$ & $0.6876_{\pm0.0103}$ & $0.7554_{\pm0.0135}$ & $0.6595_{\pm0.0433}$                        & $0.6493_{\pm0.0464}$ & $0.6882_{\pm0.0639}$ &  $0.6931_{\pm0.0120}$ &  $0.6890_{\pm0.0126}$ & $0.7192_{\pm0.0210}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & CDT                & $0.6969_{\pm0.0126}$ & $0.6841_{\pm0.0139}$ & $0.7576_{\pm0.0061}$ & $0.5873_{\pm0.0349}$                        & $0.5142_{\pm0.0493}$ & $0.6585_{\pm0.0586}$ & $0.6315_{\pm0.0103}$                        & $0.5802_{\pm0.0133}$                        & $0.7133_{\pm0.0177}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & $0.7021_{\pm0.0251}$ & $0.6938_{\pm0.0288}$ & $0.7499_{\pm0.0306}$ & $0.6774_{\pm0.0075}$                        & $0.6437_{\pm0.0120}$ & $0.6739_{\pm0.0344}$ & $0.6864_{\pm0.0064}$                        & $0.6622_{\pm0.0092}$                        & $0.7338_{\pm0.0096}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{}                            &                                            & Influence Balanced & $0.7013_{\pm0.0383}$ & $0.6961_{\pm0.0373}$ & $0.7570_{\pm0.0344}$ &  $0.6728_{\pm0.0492}$ & $0.6590_{\pm0.0561}$ & $0.7043_{\pm0.0670}$ &  $0.6943_{\pm0.0100}$ &  $0.6821_{\pm0.0103}$ & $0.7286_{\pm0.0042}$ &              &             &     &              &             &     &              &             &     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Standard}} & \multirow{-4}{*}{Module Improvement}       & BBN                & $0.6906_{\pm0.0646}$ & $0.6861_{\pm0.0697}$ & $0.7643_{\pm0.0497}$ & $0.6482_{\pm0.0328}$                        & $0.6291_{\pm0.0289}$ & $0.7225_{\pm0.0720}$ & $0.6822_{\pm0.1266}$                        & $0.6304_{\pm0.1783}$                        & $0.7298_{\pm0.1509}$ &              &             &     &              &             &     &              &             &     \\ \bottomrule
\end{tabular}
}
\end{table}

==> Tables/table-1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t]
\small
\centering
\caption{\textbf{Results for random and standard splits on 4 ImDrug classification datasets.} We perform binary classification on HIV and SBAP, and long-tailed classification on USPTO-50K and DrugBank. For each split and metric, the best method is \textbf{bolded} and the second best is \underline{underlined}.}\label{table:overall}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ccc|ccc|ccc|ccc|ccc}
\toprule
                                        \multicolumn{3}{c}{}  & \multicolumn{3}{c}{\textbf{HIV}\cite{wu2018moleculenet}}                                                                        & \multicolumn{3}{c}{\textbf{SBAP}\cite{2022arXiv220109637J}}         & \multicolumn{3}{c}{\textbf{USPTO-50K}\cite{liu2017retrosynthetic}}    & \multicolumn{3}{c}{\textbf{DrugBank}\cite{wishart2018drugbank}}     \\\midrule
\multicolumn{3}{c}{\# Graphs}                        & \multicolumn{3}{c}{41,127}                                                                     & \multicolumn{3}{c}{32,140}             & \multicolumn{3}{c}{50,036}             & \multicolumn{3}{c}{191,808}             \\
\multicolumn{3}{c}{\# Average nodes}                & \multicolumn{3}{c}{25.51}                                                                      & \multicolumn{3}{c}{32.60}             & \multicolumn{3}{c}{25.03}             & \multicolumn{3}{c}{26.43}             \\
\multicolumn{3}{c}{\# Average edges}         & \multicolumn{3}{c}{54.94}                                                                      & \multicolumn{3}{c}{103.94}             & \multicolumn{3}{c}{78.29}             & \multicolumn{3}{c}{83.21}             \\
\multicolumn{3}{c}{\# Classes}            & \multicolumn{3}{c}{2}                                                                          & \multicolumn{3}{c}{2}             & \multicolumn{3}{c}{10}             & \multicolumn{3}{c}{86}  \\           
\multicolumn{3}{c}{Imbalance ratio}            & \multicolumn{3}{c}{27.50}                                                                          & \multicolumn{3}{c}{36.77}             & \multicolumn{3}{c}{65.78}             & \multicolumn{3}{c}{216.96} 
\\ \midrule\midrule
\multicolumn{3}{c|}{Metric}                                                                                         & Balanced-Acc                          & Balanced-F1                           & AUROC            & Balanced-Acc & Balanced-F1 & AUROC & Balanced-Acc & Balanced-F1 & AUROC & Balanced-Acc & Balanced-F1 & AUROC \\ \midrule
\multicolumn{1}{c|}{}                            &                                            & Vanilla GCN       & 62.77                        & 57.39                         & 70.29 &  68.40            &     65.08        &  89.61   & 35.32      & 33.29            & 80.74     & 30.03     & 33.29     & 94.26      \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & BS  & \textbf{70.26}                        & \textbf{69.50}                        & \textbf{75.53} &   81.32          &      81.15       &  89.65   & 31.88     & 31.67    & 75.14      & \underline{50.21}    & \textbf{48.78}          &  \underline{94.31}   \\
\multicolumn{1}{c|}{}                            &                                            & CB\_F  & 66.18                        & 62.49                        & 74.11 &    74.30          &      72.78       &  90.59   & 33.18     & 32.58    & 77.77      & 35.92    & 37.73          &  91.72   \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Class- \\ rebalancing\end{tabular}}        & CS    & \underline{70.10}                        & \underline{68.92}                        & 74.33 &        \underline{83.87}      &      \underline{83.75}       &  91.29   & 40.10     & 40.17    & 81.37      & 41.82    & 43.34       & 89.63     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & Mixup              & 62.46                        & 56.70                        & 71.51 &           69.32   &      66.29       &  \underline{91.57}   & 48.26     & \underline{49.37}    & 82.84      & 30.34            & 33.31             &  93.57    \\
\multicolumn{1}{c|}{}                            &                                            & Remix              & 62.17                        & 56.24                        & 73.01 &    69.91          &      67.05       &  91.50   & \underline{49.26}     & \textbf{49.45}    & \textbf{85.79}     & 32.01              & 35.11             & \textbf{94.43}     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Information \\augmentation\end{tabular}} & DiVE               & 68.69 & 67.27 & 72.21 &         78.48     &        77.94     &   83.46    & 40.48      &  40.55           & 79.97     & 37.05 & 38.94 & 91.78  \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & CDT                & 63.31                        & 58.22                         & 72.89 &        72.83      &     71.10        &  89.69   & 35.53     & 34.85   & 78.48 & \textbf{51.74}              & \underline{46.38}             & 91.93     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & 69.43 &  67.08 & \underline{74.45} &      69.28        &       66.36      &    89.77 &  35.10        & 35.70           & 78.15     &  31.61            &  33.80           & 90.69     \\
\multicolumn{1}{c|}{}                            &                                            & IB & 68.25                        & 66.77                        & 72.99 &         77.90     &      77.71       &  86.25   & 37.31      & 37.50   & 78.69     & 45.74              & 45.17             & 93.16     \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Random}}   & \multirow{-4}{*}{\begin{tabular}{c}Module \\Improvement\end{tabular}}       & BBN                & 68.22                        & 63.04                        & 72.98 &       \textbf{88.43}       &      \textbf{88.42}       &   \textbf{92.95}  & \textbf{49.46}      & 48.81   & \underline{84.18}   &  44.26             & 44.69             & 93.32     \\ \midrule\midrule
\multicolumn{1}{c|}{}                            &                                            & Vanilla GCN       & 63.08                        & 58.01                        & 68.52 &    67.40          &  63.88           &  90.15   &  36.67      & 34.06  & 81.85   & 65.12              &    60.04         & 97.59     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & BS  & 67.30                        & 66.43                        & 72.11 &     \underline{83.24}         &      \underline{83.14}       &  91.00   & 44.81       & 44.68  & 83.35    & \textbf{89.39}             & \textbf{86.17}            & 98.02     \\
\multicolumn{1}{c|}{}                            &                                            & CB\_F  & 65.39                       & 61.43                    & \textbf{74.98} &         73.15     &       71.52      &  90.20     & 37.90          & 36.71  & 81.43  &   74.55           & 69.55             & 97.34     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Class- \\rebalancing\end{tabular}}        & CS    & \textbf{69.81}                        & \textbf{68.92}                        & \underline{74.18} &  82.61            &      82.49       & 89.64    &  42.17      & 42.10 & 82.65 &   80.48           & 75.61             & 98.10     \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & Mixup              & 63.10                        & 57.75                        & 72.40 &      68.88        &      66.01       &   \underline{91.88}  &  \underline{46.62}      & 45.71 & \textbf{85.87} &  69.41            & 65.51             & 97.80     \\
\multicolumn{1}{c|}{}                            &                                            & Remix              & 63.71                        & 58.64                        & 72.78 &      71.58        &      69.11       & 90.98    & 46.60       & \underline{45.89} & \underline{85.84}     & 72.78              & 68.99             & 97.87     \\
\multicolumn{1}{c|}{}                            & \multirow{-3}{*}{\begin{tabular}{c}Information \\augmentation\end{tabular}} & DiVE               &  69.31 &  \underline{68.90} & 71.92 &   75.07           &      74.91       & 80.00    &    44.19          & 44.61          & 83.98     & 70.24  & 64.38 & 97.73 \\\cmidrule{2-15}
\multicolumn{1}{c|}{}                            &                                            & CDT                & 63.15                       & 58.02                        & 71.33 &       67.61       &       63.98      &    89.84  & 41.22       & 39.80 & 81.98   &  81.66         & 76.62             & \textbf{98.25}     \\
\multicolumn{1}{c|}{}                            &                                            & Decoupling         & 68.64                        & 66.22                        & 73.38 &       69.58       &      66.33       &   90.99  &  39.45      & 37.84 & 82.26    & 70.24        & 67.95       & 97.74    \\
\multicolumn{1}{c|}{}                            &                                            & IB &  \underline{69.43} & 68.21 & 72.86 &     79.67         &       79.57      &    86.93  & 45.13       & 43.84  & 83.79     &    80.48          & 74.91             &  \underline{98.18}    \\
\multicolumn{1}{c|}{\multirow{-11}{*}{Standard}} & \multirow{-4}{*}{\begin{tabular}{c}Module \\Improvement\end{tabular}}       & BBN                & 68.22                        & 63.04                        & 72.98 &        \textbf{88.99}      &      \textbf{88.66}       &  \textbf{93.21}   & \textbf{49.63}       & \textbf{48.90}  & 84.39   & \underline{86.98}             & \underline{83.85}             & 98.01    \\ \bottomrule
\end{tabular}
\end{adjustbox}
% \vspace{-1em}
\end{table}

==> Tables/table-2-new.tex <==
% \begin{wraptable}{r}{9cm}
% \small
% \centering
% \vspace{-2em}
% \caption{\textbf{Results on Open LT.} The proportions of samples split into open-sets in USPTO-50K and DrugBank are 0.2 and 0.5, respectively.}\label{table:openLT}
% % For each dataset and metric, the best method is bolded and the second best is underlined.
% \vspace{1em}
% \scalebox{0.6}{
% \begin{tabular}{c|ccc|cll}
% \toprule
%                   & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
%                   & Balanced-Acc & Balanced-F1 & AUROC     & balanced-acc & \multicolumn{1}{c}{balanced-f1} & \multicolumn{1}{c}{AUROC} \\ \midrule
% Vanilla GCN      & $37.52_{\pm0.45}$   & $35.04_{\pm0.64}$  & $73.66_{\pm0.26}$ & $58.29_{\pm0.56}$   & $62.46_{\pm0.42}$                      & $96.94_{\pm0.27}$                  \\\midrule
% BS & $39.54_{\pm0.99}$   & $37.03_{\pm1.27}$  & $73.66_{\pm0.59}$  & $71.12_{\pm0.27}$   & $71.60_{\pm0.28}$                      & $97.34_{\pm0.27}$                  \\
% CB\_F & $37.28_{\pm1.36}$   & $34.62_{\pm0.71}$  & $71.94_{\pm0.65}$  & $59.75_{\pm0.39}$   & $63.26_{\pm0.78}$                      & $96.54_{\pm0.09}$                  \\
% Remix             & $48.28_{\pm0.41}$   & $45.05_{\pm0.46}$  & $76.23_{\pm0.65}$  & $69.78_{\pm0.71}$   & $72.72_{\pm0.61}$                     & $97.68_{\pm0.07}$                  \\
% IB & $39.62_{\pm0.99}$   & $33.55_{\pm2.2}$   & $69.86_{\pm0.88}$  & $62.81_{\pm0.96}$   & $64.00_{\pm0.64}$                     & $94.67_{\pm0.23}$                  \\
% BBN               & $51.30_{\pm0.35}$   & $47.82_{\pm0.31}$  & $77.05_{\pm0.29}$  & $78.75_{\pm0.52}$   & $79.36_{\pm0.25}$                      & $97.32_{\pm0.08}$                  \\ \midrule
% OLTR         & ${50.12_{\pm0.55}}$   & $47.24_{\pm0.40}$  & ${79.76_{\pm0.22}}$  & $73.55_{\pm0.34}$   & $73.54_{\pm0.29}$                      & $97.23_{\pm0.66}$                  \\
% IEM          & $51.63_{\pm0.59}$   & $48.23_{\pm0.50}$  & $\underline{80.91_{\pm0.52}}$  & $75.67_{\pm0.76}$   & $76.63_{\pm0.43}$                      & $\boldsymbol{98.09_{\pm0.23}}$                  \\ 
% OLTR+BBN   &            $\boldsymbol{60.39_{\pm0.51}}$     &  $\boldsymbol{56.09_{\pm5.20}}$                  &    $\boldsymbol{85.27_{\pm2.16}}$                            &              $\boldsymbol{82.56_{\pm5.89}}$                   &               $\boldsymbol{82.47_{\pm0.40}}$                 &                     $\underline{97.78_{\pm7.99}}$                                                                                       \\
% IEM+BBN    &          $\underline{58.63_{\pm0.42}}$                           &         $\underline{53.26_{\pm0.44}}$                       &           $80.10_{\pm3.62}$                      &            $\underline{81.80_{\pm0.67}}$                    &                  $\underline{82.13_{\pm0.46}}$                                  &    $97.58_{\pm0.53}$                                                    \\
% \bottomrule
% \end{tabular}
% }
% \end{wraptable}



  \begin{table}[t]
    \parbox{\linewidth}{
          \caption{\textbf{Results on Open LT.} The proportions of samples split into open-sets in USPTO-50K and DrugBank are 0.2 and 0.5, respectively.}\label{table:openLT}
    \begin{adjustbox}{max width=.58\textwidth}
      \centering
     \begin{tabular}{c|ccc|cll}
\toprule
                  & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
                  & Balanced-Acc & Balanced-F1 & AUROC     & Balanced-Acc & \multicolumn{1}{c}{Balanced-F1} & \multicolumn{1}{c}{AUROC} \\ \midrule
Vanilla GCN      & $85.82_{\pm0.42}$   & $81.38_{\pm0.41}$  & $94.18_{\pm0.066}$ & $91.72_{\pm0.28}$   & $91.75_{\pm0.33}$                      & $99.07_{\pm0.015}$                  \\\midrule
BS & $85.88_{\pm1.02}$   & $81.44_{\pm0.90}$  & $94.22_{\pm0.68}$  & $94.71_{\pm0.044}$   & $94.14_{\pm0.05}$                      & $99.11_{\pm0.03}$                  \\
CB\_F & $86.77_{\pm0.99}$   & $82.2_{\pm1.22}$  & $94.16_{\pm0.08}$  & $93.17_{\pm0.43}$   & $92.84_{\pm0.40}$                      & $98.80_{\pm0.11}$                  \\
Remix             & $87.92_{\pm0.23}$   & $83.40_{\pm0.21}$  & $93.91_{\pm0.13}$  & $92.68_{\pm0.83}$   & $92.75_{\pm0.59}$                     & $99.59_{\pm0.40}$                  \\
IB & $86.06_{\pm1.14}$   & $81.63_{\pm1.09}$   & $94.15_{\pm0.040}$  & $92.95_{\pm0.31}$   & $92.31_{\pm0.31}$                     & $99.03_{\pm0.04}$                  \\
BBN               & $87.86_{\pm0.14}$   & $83.32_{\pm0.13}$  & $94.07_{\pm0.19}$  & $94.52_{\pm0.33}$   & $93.96_{\pm0.34}$                      & $98.92_{\pm0.07}$                  \\ \midrule
OLTR         & ${89.21_{\pm0.75}}$   & $85.11_{\pm0.38}$  & ${96.69_{\pm0.12}}$  & $95.37_{\pm0.30}$   & $94.92_{\pm0.16}$                      & $\boldsymbol{99.79_{\pm0.09}}$                  \\
IEM          & $89.99_{\pm0.29}$   & $85.46_{\pm0.20}$  & $\underline{96.74_{\pm0.09}}$  & $95.77_{\pm0.16}$   & $95.16_{\pm0.15}$                      & $99.64_{\pm0.08}$                  \\ 
OLTR+BBN   &            $\boldsymbol{91.18_{\pm0.11}}$     &  $\boldsymbol{87.97_{\pm0.60}}$                  &    $\boldsymbol{97.72_{\pm0.56}}$                            &              $\boldsymbol{96.84_{\pm1.59}}$                   &               $\boldsymbol{96.12_{\pm0.93}}$                 &                     $\boldsymbol{99.89_{\pm0.69}}$                                                                                       \\
IEM+BBN    &          $\underline{90.66_{\pm0.41}}$                           &         $\underline{86.03_{\pm0.75}}$                       &           $96.64_{\pm1.03}$                      &            $\underline{96.06_{\pm0.76}}$                    &                  $\underline{95.59_{\pm0.96}}$                                  &    $99.77_{\pm0.12}$                                                    \\
\bottomrule
\end{tabular}
\end{adjustbox}
}

  \parbox{.42\linewidth}{
    % \vspace{0.2em}
       \caption{\textbf{Results on imbalanced regression.} We report the average performance on SBAP-Reg and QM9 in terms of mean MSE and MAE with standard deviation in this setting.}
       \label{table:ImbalancedRegression}
      \begin{adjustbox}{max width=.4\textwidth}
      \centering 
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.66_{\pm1.03}$           & $0.92_{\pm0.25}$            & $76.17_{\pm42.82}$        & $6.57_{\pm1.92}$          \\
Mixup        & $\underline{1.10_{\pm0.51}}$           & $\underline{0.78_{\pm0.17}}$            &  $82.35_{\pm36.86}$       & $6.59_{\pm1.46}$                        \\
BBN          & $1.52_{\pm1.57}$           & $0.89_{\pm0.38}$            & $\underline{59.42_{\pm14.39}}$        & $6.02_{\pm0.77}$          \\ \midrule
Focal-R       & $1.38_{\pm1.08}$           & $0.84_{\pm0.31}$            & $94.29_{\pm57.38}$        & $7.23_{\pm2.65}$          \\
LDS          & $1.36_{\pm1.16}$           & $\underline{0.78_{\pm0.26}}$            & $\boldsymbol{16.01_{\pm6.58}}$        & $\boldsymbol{2.73_{\pm0.03}}$           \\
FDS          & $\boldsymbol{0.59_{\pm0.09}}$           & $\boldsymbol{0.54_{\pm0.02}}$            & $60.81_{\pm33.52}$        & $\underline{5.63_{\pm1.53}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
}
  \end{table}

==> Tables/table-2.tex <==
% \begin{wraptable}{r}{9cm}
% \small
% \centering
% \vspace{-2em}
% \caption{\textbf{Results on Open LT.} The proportions of samples split into open-sets in USPTO-50K and DrugBank are 0.2 and 0.5, respectively.}\label{table:openLT}
% % For each dataset and metric, the best method is bolded and the second best is underlined.
% \vspace{1em}
% \scalebox{0.6}{
% \begin{tabular}{c|ccc|cll}
% \toprule
%                   & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
%                   & Balanced-Acc & Balanced-F1 & AUROC     & balanced-acc & \multicolumn{1}{c}{balanced-f1} & \multicolumn{1}{c}{AUROC} \\ \midrule
% Vanilla GCN      & $37.52_{\pm0.45}$   & $35.04_{\pm0.64}$  & $73.66_{\pm0.26}$ & $58.29_{\pm0.56}$   & $62.46_{\pm0.42}$                      & $96.94_{\pm0.27}$                  \\\midrule
% BS & $39.54_{\pm0.99}$   & $37.03_{\pm1.27}$  & $73.66_{\pm0.59}$  & $71.12_{\pm0.27}$   & $71.60_{\pm0.28}$                      & $97.34_{\pm0.27}$                  \\
% CB\_F & $37.28_{\pm1.36}$   & $34.62_{\pm0.71}$  & $71.94_{\pm0.65}$  & $59.75_{\pm0.39}$   & $63.26_{\pm0.78}$                      & $96.54_{\pm0.09}$                  \\
% Remix             & $48.28_{\pm0.41}$   & $45.05_{\pm0.46}$  & $76.23_{\pm0.65}$  & $69.78_{\pm0.71}$   & $72.72_{\pm0.61}$                     & $97.68_{\pm0.07}$                  \\
% IB & $39.62_{\pm0.99}$   & $33.55_{\pm2.2}$   & $69.86_{\pm0.88}$  & $62.81_{\pm0.96}$   & $64.00_{\pm0.64}$                     & $94.67_{\pm0.23}$                  \\
% BBN               & $51.30_{\pm0.35}$   & $47.82_{\pm0.31}$  & $77.05_{\pm0.29}$  & $78.75_{\pm0.52}$   & $79.36_{\pm0.25}$                      & $97.32_{\pm0.08}$                  \\ \midrule
% OLTR         & ${50.12_{\pm0.55}}$   & $47.24_{\pm0.40}$  & ${79.76_{\pm0.22}}$  & $73.55_{\pm0.34}$   & $73.54_{\pm0.29}$                      & $97.23_{\pm0.66}$                  \\
% IEM          & $51.63_{\pm0.59}$   & $48.23_{\pm0.50}$  & $\underline{80.91_{\pm0.52}}$  & $75.67_{\pm0.76}$   & $76.63_{\pm0.43}$                      & $\boldsymbol{98.09_{\pm0.23}}$                  \\ 
% OLTR+BBN   &            $\boldsymbol{60.39_{\pm0.51}}$     &  $\boldsymbol{56.09_{\pm5.20}}$                  &    $\boldsymbol{85.27_{\pm2.16}}$                            &              $\boldsymbol{82.56_{\pm5.89}}$                   &               $\boldsymbol{82.47_{\pm0.40}}$                 &                     $\underline{97.78_{\pm7.99}}$                                                                                       \\
% IEM+BBN    &          $\underline{58.63_{\pm0.42}}$                           &         $\underline{53.26_{\pm0.44}}$                       &           $80.10_{\pm3.62}$                      &            $\underline{81.80_{\pm0.67}}$                    &                  $\underline{82.13_{\pm0.46}}$                                  &    $97.58_{\pm0.53}$                                                    \\
% \bottomrule
% \end{tabular}
% }
% \end{wraptable}



  \begin{table}[t]
    \parbox{.58\linewidth}{
          \caption{\textbf{Results on Open LT.} The proportions of samples split into open-sets in USPTO-50K and DrugBank are 0.2 and 0.5, respectively.}\label{table:openLT}
    \begin{adjustbox}{max width=.58\textwidth}
      \centering
     \begin{tabular}{c|ccc|cll}
\toprule
                  & \multicolumn{3}{c|}{\textbf{USPTO-50K}}           & \multicolumn{3}{c}{\textbf{DrugBank}}                                                 \\ \cmidrule{2-7} 
                  & Balanced-Acc & Balanced-F1 & AUROC     & Balanced-Acc & \multicolumn{1}{c}{Balanced-F1} & \multicolumn{1}{c}{AUROC} \\ \midrule
Vanilla GCN      & $37.52_{\pm0.45}$   & $35.04_{\pm0.64}$  & $73.66_{\pm0.26}$ & $58.29_{\pm0.56}$   & $62.46_{\pm0.42}$                      & $96.94_{\pm0.27}$                  \\\midrule
BS & $39.54_{\pm0.99}$   & $37.03_{\pm1.27}$  & $73.66_{\pm0.59}$  & $71.12_{\pm0.27}$   & $71.60_{\pm0.28}$                      & $97.34_{\pm0.27}$                  \\
CB\_F & $37.28_{\pm1.36}$   & $34.62_{\pm0.71}$  & $71.94_{\pm0.65}$  & $59.75_{\pm0.39}$   & $63.26_{\pm0.78}$                      & $96.54_{\pm0.09}$                  \\
Remix             & $48.28_{\pm0.41}$   & $45.05_{\pm0.46}$  & $76.23_{\pm0.65}$  & $69.78_{\pm0.71}$   & $72.72_{\pm0.61}$                     & $97.68_{\pm0.07}$                  \\
IB & $39.62_{\pm0.99}$   & $33.55_{\pm2.2}$   & $69.86_{\pm0.88}$  & $62.81_{\pm0.96}$   & $64.00_{\pm0.64}$                     & $94.67_{\pm0.23}$                  \\
BBN               & $51.30_{\pm0.35}$   & $47.82_{\pm0.31}$  & $77.05_{\pm0.29}$  & $78.75_{\pm0.52}$   & $79.36_{\pm0.25}$                      & $97.32_{\pm0.08}$                  \\ \midrule
OLTR         & ${50.12_{\pm0.55}}$   & $47.24_{\pm0.40}$  & ${79.76_{\pm0.22}}$  & $73.55_{\pm0.34}$   & $73.54_{\pm0.29}$                      & $97.23_{\pm0.66}$                  \\
IEM          & $51.63_{\pm0.59}$   & $48.23_{\pm0.50}$  & $\underline{80.91_{\pm0.52}}$  & $75.67_{\pm0.76}$   & $76.63_{\pm0.43}$                      & $\boldsymbol{98.09_{\pm0.23}}$                  \\ 
OLTR+BBN   &            $\boldsymbol{60.39_{\pm0.51}}$     &  $\boldsymbol{56.09_{\pm5.20}}$                  &    $\boldsymbol{85.27_{\pm2.16}}$                            &              $\boldsymbol{82.56_{\pm5.89}}$                   &               $\boldsymbol{82.47_{\pm0.40}}$                 &                     $\underline{97.78_{\pm7.99}}$                                                                                       \\
IEM+BBN    &          $\underline{58.63_{\pm0.42}}$                           &         $\underline{53.26_{\pm0.44}}$                       &           $80.10_{\pm3.62}$                      &            $\underline{81.80_{\pm0.67}}$                    &                  $\underline{82.13_{\pm0.46}}$                                  &    $97.58_{\pm0.53}$                                                    \\
\bottomrule
\end{tabular}
\end{adjustbox}
}
  \parbox{.42\linewidth}{
    % \vspace{0.2em}
       \caption{\textbf{Results on imbalanced regression.} We report the average performance on SBAP-Reg and QM9 in terms of mean MSE and MAE with standard deviation in this setting.}
       \label{table:ImbalancedRegression}
      \begin{adjustbox}{max width=.4\textwidth}
      \centering 
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.99_{\pm0.52}$           & $1.13_{\pm0.14}$            & $161.55_{\pm38.18}$        & $10.40_{\pm1.39}$          \\
Mixup        & $1.34_{\pm0.18}$           & $0.92_{\pm0.17}$            &  $160.32_{\pm39.58}$       & $10.17_{\pm1.27}$                        \\
BBN          & $1.58_{\pm0.59}$           & $1.04_{\pm0.18}$            & $161.22_{\pm37.55}$        & $10.04_{\pm1.13}$          \\ \midrule
Focal-R       & $1.92_{\pm0.69}$           & $1.14_{\pm0.30}$            & $171.78_{\pm40.60}$        & $10.70_{\pm1.16}$          \\
LDS          & $\underline{1.11_{\pm0.16}}$           & $\boldsymbol{0.67_{\pm0.01}}$            & $\underline{143.15_{\pm20.69}}$        & $\underline{9.63_{\pm0.72}}$           \\
FDS          & $\boldsymbol{0.85_{\pm0.08}}$           & $\underline{0.71_{\pm0.12}}$            & $\boldsymbol{134.83_{\pm41.61}}$        & $\boldsymbol{9.28_{\pm1.51}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
}
  \end{table}

==> Tables/table-3-new.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \small
% \caption{Ablations of backbone models on USPTO-50K and USPTO-Catalyst.}\label{table:backbones}
% \scalebox{0.84}{
% \begin{tabular}{ll|lll|lll}
% \toprule
%                                   &             & \multicolumn{3}{c|}{\textbf{Random}}                    & \multicolumn{3}{c}{\textbf{Standard}}                  \\\cmidrule{3-8}
%                                   &             & Balanced-Acc  & Balanced-F1   & AUROC       & Balanced-Acc  & Balanced-F1   & AUROC       \\ \midrule
% \multirow{3}{*}{Baseline}          & Morgan      & $81.42_{\pm1.19}$ & $81.56_{\pm1.16}$ & $97.40_{\pm0.74}$ & $82.04_{\pm3.13}$ & $81.77_{\pm3.41}$ & $96.94_{\pm0.60}$ \\
%                                   & Transformer & $91.54_{\pm0.47}$ & $91.62_{\pm0.46}$ & $99.52_{\pm0.09}$ & $92.13_{\pm1.02}$ & $92.17_{\pm0.99}$ & $99.47_{\pm0.35}$ \\
%                                   & GCN    & $92.23_{\pm0.87}$ & $92.20_{\pm0.90}$ & $\underline{99.76_{\pm0.06}}$ & $92.15_{\pm0.88}$ & $92.15_{\pm0.87}$ & $99.54_{\pm0.12}$ \\ \midrule
% \multirow{3}{*}{CB\_F} & Morgan      & $81.59_{\pm0.44}$ & $81.85_{\pm0.44}$ & $95.61_{\pm0.37}$ & $81.09_{\pm4.14}$ & $81.16_{\pm4.18}$ & $94.20_{\pm0.36}$ \\
%                                   & Transformer & $91.49_{\pm0.66}$ & $91.55_{\pm0.62}$& $99.20_{\pm0.13}$ & $91.78_{\pm1.13}$ & $91.86_{\pm1.13}$ & $99.21_{\pm0.23}$ \\
%                                   & GCN    & $93.32_{\pm0.18}$ & $93.33_{\pm0.2}$ & $99.49_{\pm0.10}$ & $94.07_{\pm1.18}$ & $94.11_{\pm1.20}$ & $99.27_{\pm0.31}$ \\ \midrule
% \multirow{3}{*}{Mixup}             & Morgan      & $83.72_{\pm0.56}$ & $83.88_{\pm0.53}$ & $97.66_{\pm0.23}$ & $84.26_{\pm1.26}$ & $84.33_{\pm1.35}$ & $96.78_{\pm0.97}$ \\
%                                   & Transformer & $91.22_{\pm0.61}$ & $91.29_{\pm0.57}$ & $99.16_{\pm0.13}$ & $91.58_{\pm1.51}$ & $91.64_{\pm1.49}$ & $98.74_{\pm0.13}$ \\
%                                   & GCN    & $\underline{95.03_{\pm0.77}}$ & $\underline{95.04_{\pm0.78}}$ & $\boldsymbol{99.77_{\pm0.03}}$ & $\underline{95.21_{\pm0.37}}$
%                                     & $\underline{95.19_{\pm0.33}}$ & $\underline{99.65_{\pm0.29}}$ \\ \midrule
% \multirow{3}{*}{BBN}               & Morgan      & $83.57_{\pm1.32}$ & $83.81_{\pm1.43}$ & $97.11_{\pm0.14}$ & $85.26_{\pm2.78}$ & $85.31_{\pm2.89}$ & $97.55_{\pm0.61}$ \\
%                                   & Transformer & $89.51_{\pm0.81}$ & $89.61_{\pm0.77}$ & $98.41_{\pm0.46}$ & $88.77_{\pm2.81}$ & $89.02_{\pm2.68}$ & $98.63_{\pm0.18}$ \\
%                                   & GCN    & $\boldsymbol{95.57_{\pm0.14}}$ & $\boldsymbol{95.56_{\pm0.14}}$ & $99.67_{\pm0.03}$ & $\boldsymbol{96.23_{\pm1.35}}$ & $\boldsymbol{96.25_{\pm1.32}}$ & $\boldsymbol{99.75_{\pm0.23}}$ \\ \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[htbp]
  \centering
  \caption{Ablations of backbone models on USPTO-50K and USPTO-Catalyst. For hybrid prediction tasks/datasets, Unless otherwise specified, the training mode is single-instance prediction. USPTO-Catalyst here was formulated as multi-instance prediction.}\label{table:backbones}
  \scalebox{0.70}{
    \begin{tabular}{c|cc|ccc|ccc}
    \toprule
    \multicolumn{1}{c}{} &       &       & \multicolumn{3}{c|}{USPTO-50k} & \multicolumn{3}{c}{USPTO-Catalyst} \\
    \multicolumn{1}{c}{} &       &       & Balanced-Acc & Balanced-F1 & AUROC & Balanced-Acc & Balanced-F1 & AUROC \\
    \midrule
    \midrule
    \multirow{12}[8]{*}{Random} & \multirow{3}[2]{*}{Baseline} & Morgan &$81.42_{\pm1.19}$ & $81.56_{\pm1.16}$ & $97.40_{\pm0.74}$ & $14.62_{\pm0.49}$ & $16.57_{\pm0.58}$ & $87.65_{\pm0.21}$  \\
          &       & Transformer &$91.54_{\pm0.47}$ & $91.62_{\pm0.46}$ & $99.52_{\pm0.09}$ &$17.11_{\pm1.34}$ & $17.08_{\pm3.84}$ & $\boldsymbol{94.72_{\pm0.21}}$  \\
          &       & GCN   & $92.23_{\pm0.87}$ & $92.20_{\pm0.90}$ & $\underline{99.76_{\pm0.06}}$ & $16.33_{\pm0.56}$ & $15.85_{\pm2.15}$ & $92.81_{\pm0.41}$  \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{CB\_F} & Morgan & $81.59_{\pm0.44}$ & $81.85_{\pm0.44}$ & $95.61_{\pm0.37}$ & $13.14_{\pm1.44}$ & $14.67_{\pm1.52}$ & $85.82_{\pm0.27}$  \\
          &      & Transformer &$91.49_{\pm0.66}$ & $91.55_{\pm0.62}$& $99.20_{\pm0.13}$ & $17.98_{\pm0.38}$ & $18.17_{\pm0.45}$ & $90.45_{\pm0.08}$  \\
          &       & GCN   & $93.32_{\pm0.18}$ & $93.33_{\pm0.2}$ & $99.49_{\pm0.10}$ & $\underline{21.36_{\pm0.61}}$ & $\boldsymbol{23.09_{\pm0.72}}$ & $90.56_{\pm0.10}$  \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{Mixup} & Morgan & $83.72_{\pm0.56}$ & $83.88_{\pm0.53}$ & $97.66_{\pm0.23}$ & $15.41_{\pm0.3}$ & $16.39_{\pm0.36}$ & $89.38_{\pm0.17}$  \\
          &      & Transformer & $91.22_{\pm0.61}$ & $91.29_{\pm0.57}$ & $99.16_{\pm0.13}$ & $12.86_{\pm0.18}$ & $12.57_{\pm0.19}$ & $\underline{94.34_{\pm0.06}}$  \\
          &       & GCN   &$\underline{95.03_{\pm0.77}}$ & $\underline{95.04_{\pm0.78}}$ & $\boldsymbol{99.77_{\pm0.03}}$ & $16.95_{\pm0.56}$ & $18.69_{\pm0.69}$& $94.11_{\pm0.09}$ \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{BBN} & Morgan & $83.57_{\pm1.32}$ & $83.81_{\pm1.43}$ & $97.11_{\pm0.14}$ & $18.30_{\pm0.65}$ & $21.18_{\pm0.66}$ & $83.59_{\pm0.39}$  \\
          &       & Transformer & $89.51_{\pm0.81}$ & $89.61_{\pm0.77}$ & $98.41_{\pm0.46}$ & $9.71_{\pm8.32}$ & $9.03_{\pm7.83}$ & $76.53_{\pm22.26}$  \\
          &       & GCN   &  $\boldsymbol{95.57_{\pm0.14}}$ & $\boldsymbol{95.56_{\pm0.14}}$ & $99.67_{\pm0.03}$ & $\boldsymbol{22.27_{\pm1.73}}$ & $\underline{22.70_{\pm1.40}}$ & $89.08_{\pm1.86}$  \\
    \midrule
    \midrule
    \multirow{12}[8]{*}{Standard} & \multirow{3}[2]{*}{Baseline} & Morgan & $82.04_{\pm3.13}$ & $81.77_{\pm3.41}$ & $96.94_{\pm0.60}$ & $13.89_{\pm0.17}$ & $12.96_{\pm1.95}$ & $87.79_{\pm0.73}$  \\
          &       & Transformer &  $92.13_{\pm1.02}$ & $92.17_{\pm0.99}$ & $99.47_{\pm0.35}$  & $16.66_{\pm0.90}$ & $15.68_{\pm2.40}$ & $\boldsymbol{94.97_{\pm0.36}}$  \\
          &       & GCN   & $92.15_{\pm0.88}$ & $92.15_{\pm0.87}$ & $99.54_{\pm0.12}$& $16.33_{\pm0.56}$ & $15.85_{\pm2.15}$ & $92.81_{\pm0.41}$  \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{CB\_F} & Morgan &  $81.09_{\pm4.14}$ & $81.16_{\pm4.18}$ & $94.20_{\pm0.36}$ & $12.51_{\pm0.56}$ & $11.76_{\pm1.43}$ & $86.48_{\pm0.47}$  \\
          &       & Transformer &  $91.78_{\pm1.13}$ & $91.86_{\pm1.13}$ & $99.21_{\pm0.23}$  & $18.26_{\pm0.72}$ & $16.48_{\pm1.50}$ & $91.19_{\pm0.51}$  \\
          &       & GCN   & $94.07_{\pm1.18}$ & $94.11_{\pm1.20}$ & $99.27_{\pm0.31}$ & $\underline{21.68_{\pm0.28}}$ & $\underline{20.51_{\pm1.93}}$ & $90.82_{\pm0.40}$  \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{Mixup} & Morgan & $84.26_{\pm1.26}$ & $84.33_{\pm1.35}$ & $96.78_{\pm0.97}$ & $14.86_{\pm0.10}$  & $13.45_{\pm1.37}$ & $89.50_{\pm0.49}$  \\
          &      & Transformer &$91.58_{\pm1.51}$ & $91.64_{\pm1.49}$ & $98.74_{\pm0.13}$  & $12.41_{\pm0.17}$  & $10.45_{\pm0.89}$ & $\underline{94.90_{\pm0.27}}$  \\
          &       & GCN   &$\underline{95.21_{\pm0.37}}$ & $\underline{95.19_{\pm0.33}}$ & $\underline{99.65_{\pm0.29}}$ & $16.62_{\pm1.03}$ & $15.50_{\pm2.28}$ & $94.38_{\pm0.28}$  \\
\cmidrule{2-9}          & \multirow{3}[2]{*}{BBN} & Morgan &  $85.26_{\pm2.78}$ & $85.31_{\pm2.89}$ & $97.55_{\pm0.61}$ & $17.04_{\pm1.69}$ & $16.5_{\pm3.40}$ & $86.30_{\pm0.37}$  \\
          &       & Transformer &$88.77_{\pm2.81}$ & $89.02_{\pm2.68}$ & $98.63_{\pm0.18}$& $14.25_{\pm2.14}$ & $12.19_{\pm2.91}$ & $91.36_{\pm1.12}$  \\
          &       & GCN   & $\boldsymbol{96.23_{\pm1.35}}$ & $\boldsymbol{96.25_{\pm1.32}}$ & $\boldsymbol{99.75_{\pm0.23}}$  & $\boldsymbol{21.79_{\pm0.96}}$ & $\boldsymbol{20.61_{\pm1.69}}$ & $91.18_{\pm1.70}$  \\
    \bottomrule
    \end{tabular}%
    }
\end{table}%


==> Tables/table-3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\small
\caption{Ablations of backbone models on USPTO-50K.}\label{table:backbones}
\scalebox{0.84}{
\begin{tabular}{ll|lll|lll}
\toprule
                                   &             & \multicolumn{3}{c|}{\textbf{Random}}                    & \multicolumn{3}{c}{\textbf{Standard}}                  \\\cmidrule{3-8}
                                   &             & Balanced-Acc  & Balanced-F1   & AUROC       & Balanced-Acc  & Balanced-F1   & AUROC       \\ \midrule
\multirow{3}{*}{Baseline}          & Morgan      & $19.40_{\pm0.89}$ & $13.61_{\pm0.59}$ & $68.04_{\pm1.68}$ & $18.89_{\pm0.97}$ & $13.32_{\pm0.66}$ & $66.95_{\pm1.24}$ \\
                                   & Transformer & $32.26_{\pm1.84}$ & $31.77_{\pm2.42}$ & $78.64_{\pm0.39}$ & $32.82_{\pm2.26}$ & $31.06_{\pm2.47}$ & $78.48_{\pm1.68}$ \\
                                   & GCN    & $35.32_{\pm2.27}$ & $33.29_{\pm1.23}$ & $80.74_{\pm3.10}$ & $36.67_{\pm0.56}$ & $34.06_{\pm0.18}$ & $81.85_{\pm2.01}$ \\ \midrule
\multirow{3}{*}{CB\_F} & Morgan      & $22.09_{\pm0.48}$ & $17.67_{\pm0.50}$ & $68.57_{\pm1.90}$ & $21.59_{\pm2.03}$ & $17.24_{\pm1.17}$ & $68.69_{\pm1.31}$ \\
                                   & Transformer & $34.91_{\pm1.70}$ & $35.36_{\pm1.88}$& $76.94_{\pm0.32}$ & $35.10_{\pm2.04}$ & $34.45_{\pm2.30}$ & $78.22_{\pm0.55}$ \\
                                   & GCN    & $33.18_{\pm1.70}$ & $32.58_{\pm1.83}$ & $77.77_{\pm2.25}$ & $37.90_{\pm2.51}$ & $36.71_{\pm2.11}$ & $81.43_{\pm1.29}$ \\ \midrule
\multirow{3}{*}{Remix}             & Morgan      & $26.40_{\pm1.90}$ & $21.40_{\pm2.46}$ & $68.88_{\pm0.77}$ & $16.79_{\pm0.60}$ & $10.85_{\pm0.18}$ & $65.59_{\pm1.26}$ \\
                                   & Transformer & $40.33_{\pm0.94}$ & $41.16_{\pm0.91}$ & $78.41_{\pm0.08}$ & $31.47_{\pm0.94}$ & $29.74_{\pm1.06}$ & $78.56_{\pm0.52}$ \\
                                   & GCN    & $\underline{49.26_{\pm0.24}}$ & $\boldsymbol{49.45_{\pm1.54}}$ & $\boldsymbol{85.79_{\pm2.65}}$ & $\underline{46.60_{\pm3.59}}$
                                    & $\underline{45.89_{\pm4.57}}$ & $\boldsymbol{85.84_{\pm1.65}}$ \\ \midrule
\multirow{3}{*}{BBN}               & Morgan      & $17.13_{\pm2.33}$ & $8.37_{\pm1.75}$ & $61.77_{\pm4.60}$ & $16.30_{\pm1.70}$ & $7.50_{\pm1.04}$ & $63.73_{\pm5.64}$ \\
                                   & Transformer & $35.92_{\pm6.41}$ & $31.20_{\pm9.77}$ & $77.96_{\pm0.29}$ & $34.07_{\pm8.48}$ & $31.46_{\pm9.56}$ & $73.93_{\pm7.13}$ \\
                                   & GCN    & $\boldsymbol{49.46_{\pm3.62}}$ & $\underline{48.81_{\pm2.26}}$ & $\underline{84.18_{\pm2.33}}$ & $\boldsymbol{49.63_{\pm3.39}}$ & $\boldsymbol{48.90_{\pm2.14}}$ & $\underline{84.39_{\pm2.13}}$ \\ \bottomrule
\end{tabular}
}
\end{table}

==> Tables/table-4-new.tex <==
% \begin{wraptable}[9]{r}{7.5cm}
\begin{table}[tbh]
\vspace{-2em}
\caption{\textbf{Results on imbalanced regression.} }\label{table:ImbalancedRegression}
\vspace{1em}
\small
\centering
\begin{adjustbox}{max width=0.5\textwidth}
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.99_{\pm0.52}$           & $1.13_{\pm0.14}$            & $161.55_{\pm38.18}$        & $10.40_{\pm1.39}$          \\
Mixup        & $1.34_{\pm0.18}$           & $0.92_{\pm0.17}$            &  $160.32_{\pm39.58}$       & $10.17_{\pm1.27}$                        \\
BBN          & $1.58_{\pm0.59}$           & $1.04_{\pm0.18}$            & $161.22_{\pm37.55}$        & $10.04_{\pm1.13}$          \\ \midrule
Focal\_R       & $1.92_{\pm0.69}$           & $1.14_{\pm0.30}$            & $171.78_{\pm40.60}$        & $10.70_{\pm1.16}$          \\
LDS          & $\underline{1.11_{\pm0.16}}$           & $\boldsymbol{0.67_{\pm0.01}}$            & $\underline{143.15_{\pm20.69}}$        & $\underline{9.63_{\pm0.72}}$           \\
FDS          & $\boldsymbol{0.85_{\pm0.08}}$           & $\underline{0.71_{\pm0.12}}$            & $\boldsymbol{134.83_{\pm41.61}}$        & $\boldsymbol{9.28_{\pm1.51}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \end{wraptable}

==> Tables/table-4.tex <==
% \begin{wraptable}[9]{r}{7.5cm}
\begin{table}[tbh]
\vspace{-2em}
\caption{\textbf{Results on imbalanced regression.} }\label{table:ImbalancedRegression}
\vspace{1em}
\small
\centering
\begin{adjustbox}{max width=0.5\textwidth}
\begin{tabular}{c|cc|cc}
\toprule
             & \multicolumn{2}{c|}{\textbf{SBAP-Reg}}                      & \multicolumn{2}{c}{\textbf{QM9}}                           \\ \cmidrule{2-5} 
             & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c|}{MAE} & \multicolumn{1}{c}{MSE} & \multicolumn{1}{c}{MAE} \\ \midrule
Vanilla GCN & $1.99_{\pm0.52}$           & $1.13_{\pm0.14}$            & $161.55_{\pm38.18}$        & $10.40_{\pm1.39}$          \\
Mixup        & $1.34_{\pm0.18}$           & $0.92_{\pm0.17}$            &  $160.32_{\pm39.58}$       & $10.17_{\pm1.27}$                        \\
BBN          & $1.58_{\pm0.59}$           & $1.04_{\pm0.18}$            & $161.22_{\pm37.55}$        & $10.04_{\pm1.13}$          \\ \midrule
Focal\_R       & $1.92_{\pm0.69}$           & $1.14_{\pm0.30}$            & $171.78_{\pm40.60}$        & $10.70_{\pm1.16}$          \\
LDS          & $\underline{1.11_{\pm0.16}}$           & $\boldsymbol{0.67_{\pm0.01}}$            & $\underline{143.15_{\pm20.69}}$        & $\underline{9.63_{\pm0.72}}$           \\
FDS          & $\boldsymbol{0.85_{\pm0.08}}$           & $\underline{0.71_{\pm0.12}}$            & $\boldsymbol{134.83_{\pm41.61}}$        & $\boldsymbol{9.28_{\pm1.51}}$           \\\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}
% \end{wraptable}
